Large Language Models as Evaluators for Recommendation Explanations

The explainability of recommender systems has attracted significant attention in academia and industry. Many efforts have been made for explainable recommendations, yet evaluating the quality of the explanations remains a challenging and unresolved issue. In recent years, leveraging LLMs as evaluators presents a promising avenue in Natural Language Processing tasks (e.g., sentiment classification, information extraction), as they perform strong capabilities in instruction following and common-sense reasoning. However, evaluating recommendation explanatory texts is different from these NLG tasks, as its criteria are related to human perceptions and are usually subjective. In this paper, we investigate whether LLMs can serve as evaluators of recommendation explanations. To answer the question, we utilize real user feedback on explanations given from previous work and additionally collect third-party annotations and LLM evaluations. We design and apply a 3-level meta evaluation strategy to measure the correlation between evaluator labels and the ground truth provided by users. Our experiments reveal that LLMs, such as GPT4, can provide comparable evaluations with appropriate prompts and settings. We also provide further insights into combining human labels with the LLM evaluation process and utilizing ensembles of multiple heterogeneous LLM evaluators to enhance the accuracy and stability of evaluations. Our study verifies that utilizing LLMs as evaluators can be an accurate, reproducible and cost-effective solution for evaluating recommendation explanation texts. Our code is available at https://github.com/Xiaoyu-SZ/LLMasEvaluator.

==> 4-experiment.tex <==
% \section{Experiments}
% \label{sec:experiment}

% This section presents experimental results and analyses of \shortname~ on two large public datasets. We empirically discuss the effectiveness  and explainability of our proposed method and answer the following questions: 

% \textbf{RQ1}: Does our proposed model outperform previous neural logical recommendation models and recommendation baselines?

% \textbf{RQ2}: How do our proposed modules and the hyper-parameters influence the model's performance? 

% \textbf{RQ3}: Can our proposed model provide explainable results based on the input features?
% %\end{enumerate}

% To answer \textbf{RQ1}, we conduct experiments on two large datasets and report the overall performances of our proposed model and baselines in Section \ref{sec:overall_performance}. For \textbf{RQ2}, we report the ablation study and parameter analysis of our proposed model in Sections \ref{sec:ablation} and \ref{sec:parameter_analysis}. And for \textbf{RQ3}, we report several representative cases generated by our proposed method in Section \ref{sec:casestudy}.

% \subsection{Experimental Settings}
% \subsubsection{Datasets}
% \begin{table}[htbp]
% \vspace{-2mm}
%   \caption{Statistics of the datasets. UserID and ItemID is excluded in \#Feature.}
%   \label{tab:datasets}
%   \vspace{-2mm}
%   \begin{tabular}{p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}}
%     \toprule
%     Dataset & \#User & \#User Feature & \#Item & \#Item Feature & \#Interaction \\
%     \midrule
%     \textbf{RSC2017} & 1,497,020 & 11 & 1,306,054 & 10 & 6,470,857 \\
%     \textbf{Taobao} & 1,061,769 & 8 & 846,812 & 5 &21,567,526 \\
%   \bottomrule
% \end{tabular}
% % \vspace{-5mm}
% \end{table}

%  \begin{table*}[t!]
%   \caption{The performance on two datasets. 
%   % $\lambda_r$ is the coefficient of the logical terms in the loss function. 
%   Underlines(\underline{N}) show the best results among all baselines and bold fonts (\textbf{N}) are for the overall best result. Star(*) indicates that the performance is significantly better than the best of baselines (\underline{N}) with $p<0.05$.}
%   \label{tab:performance_rec}
%   \centering
%   % \small what is this
%   \begin{tabular}{p{1cm} p{3.2cm}ccc ccc ccc ccc }
%     \toprule
%     \multicolumn{2}{c}{}&
%     \multicolumn{3}{c}{\textbf{Persuasiveness}}&
%     \multicolumn{3}{c}{\textbf{Transparency}} &
%     \multicolumn{3}{c}{\textbf{Accuracy}} &
%     \multicolumn{3}{c}{\textbf{Satisfaction}}
%     \\
%     \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}

%     &  & r & $\rho$ & $\tau$ & r & $\rho$ & $\tau$ & r & $\rho$ & $\tau$ & r & $\rho$ & $\tau$ \\
%     \cmidrule(lr){1-2}\cmidrule(lr){3-14}
%     \multirow{4}{*}{\parbox{0.5cm}{Dataset Level}}& BLEU-1 & 11.68 & 10.30 & 7.68& 10.06 & 8.59 & 6.46& 6.43 & 4.66 & 3.46& 11.36 & 9.11 & 6.82 \\
%     & BLEU-4 & -1.17 & -2.28 & -1.74& -3.47 & -3.39 & -2.58& -4.63 & -6.26 & -4.80& 0.61 & -0.69 & -0.52 \\
%     & ROUGE-L & 14.16 & 12.67 & 9.62& 11.93 & 10.65 & 8.13& 8.61 & 6.95 & 5.31& 12.87 & 10.63 & 8.12 \\
%     % & BertScore& 20.43 & 20.48 & 15.38& 18.99 & 19.38 & 14.56& \textbf{22.65} & \textbf{23.03} & 17.67& \textbf{24.96} & 23.18 & 17.62 \\

%     \cmidrule(lr){2-14}
%     & Annotator (1)& 22.44 & 23.21 & 19.28& 8.24 & 9.13 & 8.15& 7.33 & 8.50 & 7.24& 15.71 & 18.50 & 15.49 \\

%     & Annotator (2) & 18.07 & 19.00 & 15.90& \textbf{27.97} & 33.19 & 30.06& 4.88 & 3.22 & 2.51& -1.35 & 2.38 & 1.53 \\
    
%     & Annotator (Average) & 24.49 & 25.13 & 20.12& 20.52 & \textbf{26.38} & \textbf{22.86}& 7.82 & 8.76 & 7.24& 8.60 & 12.09 & 9.74 \\

%     \cmidrule(lr){2-14}
    
%     & GPT3.5-SingleAspect& 26.81 & \textbf{28.76} & 23.99& \textbf{20.62} & 21.70 & 17.98& 16.33 & 17.95 & 15.15& (9.95 & 7.83 & 6.74)  \\
%     & GPT3.5-MultipleAspect & 26.41 & 28.19 & 23.96& 11.16 & 10.67 & 9.05& 12.09 & 13.16 & 10.98& 20.93 & 21.86 & 18.51\\
%     & GPT4-SingleAspect & 18.17 & 23.30 & 19.80& 16.94 & 17.36 & 14.99& 17.55 & 15.79 & 13.66& (9.50 & 3.76 & 3.26) \\
%     & GPT4-MultipleAspect & \textbf{27.26} & 28.15 & \textbf{24.25}& 12.68 & 13.01 & 11.33& \textbf{20.30} & \textbf{22.15} & \textbf{19.45}& 24.05 & \textbf{26.24} & \textbf{22.90} \\

%     %====================
%     \midrule
%     \midrule
    
%     \multirow{4}{*}{\parbox{0.5cm}{User Level}}&  BLEU-1 & 15.84 & 12.87 & 9.83& 12.69 & 9.40 & 7.13& 10.71 & 7.76 & 5.97& 12.91 & 9.42 & 6.97 \\
%     & BLEU-4 & 7.68 & 7.01 & 5.41& 4.13 & 3.52 & 2.71& 4.80 & 4.17 & 3.34& 6.86 & 6.35 & 4.95 \\
%     & ROUGE-L & 16.39 & 13.63 & 10.60& 12.74 & 10.22 & 7.91& 11.02 & 8.49 & 6.67& 13.20 & 10.19 & 7.74 \\
%     % & BertScore & 23.00 & 22.39 & 17.45& 20.69 & 21.37 & 16.60& 24.90 & 25.18 & 19.78& 26.71 & 24.52 & 19.12 \\
    
%     \cmidrule(lr){2-14}

%     & Annotator (1) & 20.57 & 21.76 & 18.30& 7.42 & 7.05 & 6.51& 7.21 & 8.07 & 7.14& 15.56 & 16.68 & 14.03 \\

%     & Annotator (2) & 17.26 & 17.88 & 15.26& 27.44 & 30.49 & 28.07& 3.48 & 2.28 & 1.77& 1.42 & 1.70 & 0.96 \\
    
%     & Annotator (Average) & 22.97 & 23.81 & 19.25& 20.27 & 22.77 & 20.28& 7.41 & 8.07 & 6.99& 10.44 & 11.80 & 9.64 \\

%     \cmidrule(lr){2-14}
    

%     & GPT3.5-SingleAspect & 26.36 & 27.74 & 23.53& 21.22 & 22.06 & 18.82& 15.56 & 16.64 & 14.25& 7.75 & 5.70 & 4.91 \\
%     & GPT3.5-MultipleAspect & 26.36 & 27.06 & 23.31& 9.86 & 9.45 & 8.13& 10.63 & 11.29 & 9.56& 19.56 & 19.76 & 16.99 \\
%     & GPT4-SingleAspect & 19.37 & 24.03 & 20.88& 17.76 & 17.83 & 15.80& 19.32 & 15.80 & 14.03& 7.40 & 2.55 & 2.16 \\
%     & GPT4-MultipleAspect & 28.25 & 28.59 & 25.06& 12.17 & 12.85 & 11.32& 22.04 & 23.92 & 21.34& 25.12 & 26.56 & 23.63 \\

%     %====================
%     \midrule
%     \midrule
%     \multirow{4}{*}{\parbox{0.5cm}{Pair Level}}& BLEU-1 & 17.07 & 14.25 & 12.17& 14.44 & 11.59 & 10.01& 12.18 & 9.18 & 7.97& 15.79 & 13.03 & 11.23 \\
%     & BLEU-4 & 13.53 & 12.69 & 10.82& 10.24 & 9.79 & 8.51& 8.96 & 7.69 & 6.75& 12.09 & 10.67 & 9.17 \\
%     & ROUGE-L & 17.56 & 13.69 & 11.52& 14.45 & 10.85 & 9.23& 12.83 & 7.78 & 6.60& 16.23 & 11.00 & 9.26\\
%     % & BertScore & 26.27 & 24.77 & 21.07& 26.24 & 26.24 & 22.36& 29.05 & 29.15 & 24.99& 30.02 & 27.34 & 22.67 \\
    
%     \cmidrule(lr){2-14}

%     & Annotator (1) & 20.22 & 21.79 & 19.49& 5.18 & 5.70 & 5.32& 6.66 & 7.37 & 6.96& 12.62 & 13.36 & 11.59 \\

%     & Annotator (2) & 21.59 & 22.31 & 19.65& 31.39 & 33.70 & 31.84& 2.80 & 1.89 & 1.48& 0.22 & 0.76 & -0.05 \\
    
%     & Annotator (Average) & 25.28 & 25.95 & 21.94& 19.67 & 24.68 & 23.05& 6.03 & 7.49 & 7.01& 7.75 & 9.21 & 7.51 \\

%     \cmidrule(lr){2-14}
    
%     & GPT3.5-SingleAspect & 29.58 & 29.17 & 26.12& 25.01 & 24.42 & 22.17& 17.93 & 18.14 & 16.10& 6.33 & 5.80 & 5.08 \\
%     & GPT3.5-MultipleAspect  & 28.20 & 28.47 & 25.74& 11.38 & 11.01 & 9.72& 11.15 & 11.09 & 9.83& 20.78 & 20.91 & 18.75 \\
%     & GPT4-SingleAspect & 27.90 & 26.21 & 24.02& 17.64 & 17.58 & 15.95& 16.97 & 16.46 & 14.67& 6.23 & 4.30 & 3.76  \\
%     & GPT4-MultipleAspect & 28.99 & 29.70 & 27.04& 13.26 & 14.01 & 12.80& 24.93 & 25.55 & 23.62& 27.35 & 28.28 & 26.03 \\
    

    
%   \bottomrule
% \end{tabular}

% % \begin{minipage}{12cm}
% %   \begin{tablenotes}
% %   \item 
% %   \end{tablenotes}
% % \end{minipage}
% \end{table*}

% We conduct experiments on two large public datasets, i.e., \textbf{RSC2017}\footnote{\url{https://recsys.acm.org/recsys17/challenge/}} and \textbf{Taobao}\footnote{https://tianchi.aliyun.com/dataset/dataDetail?dataId=56}.
% These datasets contain millions of users, items, and interactions of two different scenarios, namely job recommendation and advertisement recommendation. 
% Statistics of two datasets are shown in Table \ref{tab:datasets}. 

% The dataset \textbf{RSC2017} is from ACM Recsys Challenge 2017, provided by \emph{XING}, a social network for business. The dataset contains rich feature information about user-job interaction. 
% The density of the dataset is 0.0003\%.
% \textbf{Taobao} is a dataset of click rate prediction about display advertisement provided by \emph{Alibaba}. 
% The density of the dataset is 0.002\%.
% %We retain the latest one when removing duplicate interactions. 

% %Further details of the datasets are introduced as follows:
% \subsubsection{Baselines}
% % We compare our model with three kinds of baselines: collaborative filtering models, feature-enhanced models, continuous neural reasoning models and discrete neural reasoning models.
% To show the effectiveness of our proposed model \shortname, we mainly select classical collaborative filtering model \textbf{BiasedMF}~\cite{RendleMF2012}, content-aware models \textbf{FM}~\cite{RendleFM2020}, \textbf{Wide\&Deep}~\cite{RecSysWideDeep2016}, and \textbf{DeepFM}~\cite{IJCAIDeepFM2017}
% , explainable recommendation model \textbf{AFM}~\cite{DBLP:AFM} and \textbf{XGBoost}~\cite{KDD16XGBoost}, and state-of-the-art neural logical recommendation model \textbf{LTNRec}~\cite{LTNForRec2022Tommaso}, \textbf{NLR}~\cite{cikm2020LINN}, \textbf{NCR}~\cite{ChenNCR2021}, and \textbf{NS-ICF}~\cite{ZhangNSICF2022} as the baseline models. 
% %All models use BPR~\cite{RendleMF2012} loss without additional specifications. 
% %The involved models are listed as follows: 
% %\begin{itemize}

% \textbf{BiasedMF}~\cite{RendleMF2012} is a matrix factorization method that acquires predictions of user\&item id embeddings. 
% %The embedding vectors are trained by existing interaction records without using feature information.
% %\textbf{FM}~\cite{RendleFM2020} is a content-aware recommendation method that models the second-order interaction between features.\textbf{Wide\&Deep}~\cite{RecSysWideDeep2016} is a content-aware recommendation model that consists of a deep neural network and a wide linear network.\textbf{DeepFM}~\cite{IJCAIDeepFM2017} is a content-aware recommendation model that consists of a deep neural network and a factorization machine.
% \textbf{Wide\&Deep}~\cite{RecSysWideDeep2016} qq and \textbf{DeepFM}~\cite{IJCAIDeepFM2017} can be treated as the advanced version of \textbf{FM}~\cite{RendleFM2020} with complex and effective neural network modules. 
% \textbf{AFM}~\cite{DBLP:AFM} is a content-aware recommendation model that utilizes attention distributions to provide explanations.
% % \item \textbf{DCNV2}
% \textbf{XGBoost}~\cite{KDD16XGBoost} is a widely used explainable machine learning method that is based on the ensemble of decision trees.
% \textbf{LTNRec}~\cite{LTNForRec2022Tommaso} is a neural logical recommendation model that employs LTN~\cite{LTN2016Luciano} on recommendation. The framework allows the injection of predefined external knowledge. It employs a logic loss based on MSE loss, so we add \textbf{BiasedMF+MSE} for comparison.
% %\item 
% %\item 
% \textbf{NLR}~\cite{cikm2020LINN} is a neural logical reasoning method that uses logic-integrated modules to learn interaction lists of users.
% %\item 
% \textbf{NCR}~\cite{ChenNCR2021} is a neural collaborative reasoning method that uses logic-integrated modules to learn user\&item interaction.
% \textbf{NS-ICF}~\cite{ZhangNSICF2022} is an interpretable collaborative filtering method that learns decision rule sets of one-hot encoded features. 

% %\end{itemize}
% \subsubsection{Evaluation Metrics}
% To evaluate the effectiveness of our proposed model, we utilize the famous ranking-based metrics~\cite{DBLP:conf/recsys/evaluation1}
% %Since the model is designed for Top-K recommendation, we use 
% NDCG@$K$ (Normalized Discounted Cumulative Gain) and HR@$K$~  (Hit Rate), and the K is set to 5 and 10 in the experiments. %in which NDCG@10 is used for validation and NDCG@5, NDCG@10, HR@10 are used for test. 
% We use real-plus-N strategy for evaluation~\cite{ZhaoExpSetCIKM2020}. 
% 1,000 irrelevant items are sampled and ranked with the real interaction together when calculating the metrics.

% \subsubsection{Paramater Settings}
% We adopt the leave-one-out strategy to split the dataset into training, validating, and testing~\cite{ZhaoExpSetCIKM2020}. The last two interactions of each user in time order separately into the validation and test sets. Each user in the testing set has at least one interaction in the training set. 
% For all models, the batch size is fixed to 128, and the size of embedding vectors is set to 64. We use an Adam optimizer with a learning rate of 1e-3, and the dropout rate is 0.2. The weight of $l2$ regularizers ($\lambda_{theta}$ in Section \ref{sec:Loss}) is tuned from 0 to 1e-5 on a log scale. No improvement in validation metrics after 20 epochs will bring the training to an early stop.
% For hyper-parameters in \shortname, the weight of logic regularizers in loss function ($\lambda_r$ in Section \ref{sec:Loss}) is searched in $\{$0, 1e-8, 1e-7, 1e-6, 1e-5, 1e-4$\}$. 
% The default value of $\lambda_{r}$ is 1e-8 for RSC2017 and 1e-6 for Taobao. 
% The number of disjunction/conjunction rules learned respectively in the model is searched in $\{$4, 8, 12, 16, 32$\}$ and set to 16 without extra statements. 

% % \begin{table}[]
% %  \vspace{-1mm}
% %   \caption{Ablation study of certain modules on \shortname. The bold font(\textbf{N}) marks the best result within a column.}
% %   \label{tab:ablation}
% %   \centering
% %   \small
% %   \begin{tabular}{l|lll}
% %     \toprule
% %     \multicolumn{1}{c}{}&
% %     \multicolumn{3}{c}{\textbf{RSC2017}}\\
% %     \cmidrule(lr){2-4} 
% %      & NDCG@5 & NDCG@10 & HR@10 \\
% %     \midrule
% %     FENCR& \textbf{0.5579}  &   \textbf{0.5797}   &  \textbf{ 0.6941}   \\
% %     % &   \textbf{0.3996}   &  \textbf{0.5837}\\
% %     w/o Selector & 0.5506 &   0.5724   &  0.6874 \\
% %     %&   0.3932   &  0.5751 \\
% %     w/o LR & 0.5520  & 0.5748   &  0.6918  \\
% %     %&   0.3946  &  0.5764 \\
% %     \midrule
% %     \midrule
% %     \multicolumn{1}{c}{}&
% %     \multicolumn{3}{c}{\textbf{Taobao}}\\
% %     \cmidrule(lr){2-4} 
% %      & NDCG@5 & NDCG@10 & HR@10 \\
% %     \midrule
% %     FENCR & \textbf{0.3653} &   \textbf{0.3996}   &  \textbf{0.5837}\\
% %     w/o Selector & 0.3603 & 0.3932   &  0.5751 \\
% %     w/o LR &  0.3608 &   0.3946  &  0.5764 \\
% %     % U-F Only & 0.5478 & 0.6474 & 0.3363 & 0.4991 \\
% %     % I-F Only & 0.5389 & 0.6549 & 0.3938 & 0.5679 \\   
% %     % U-S Voting  &   0.5669   &   0.6862   &   0.3861   &   0.5720\\
% %     % I-S Voting &   0.5748   &   0.6899   &   0.3908   &   0.5743\\
% %     % C-W Voting &   0.5545   &   0.6772   &   0.3773   &   0.5684\\

% %   \bottomrule
% % \end{tabular}
% % \end{table}

% \begin{table}[]
%  \vspace{-1mm}
%   \caption{Ablation study of certain modules on \shortname. The bold font(\textbf{N}) marks the best result within a column.}
%   \vspace{-1mm}
%   \label{tab:ablation}
%   \centering
%   \small
%   \begin{tabular}{l|ll|ll}
%     \toprule
%     \multicolumn{1}{c}{}&
%     \multicolumn{2}{c}{\textbf{RSC2017}} &
%     \multicolumn{2}{c}{\textbf{Taobao}}
%     \\
%     \cmidrule(lr){2-5} 
%      & NDCG@10 & HR@10 & NDCG@10 & HR@10 \\
%     \midrule
%     FENCR& \textbf{0.5797}  &  \textbf{ 0.6941}  & \textbf{0.3996}   &  \textbf{0.5837} \\
%     w/o Feature Selector & 0.5724 &   0.6874   &   0.3932   &  0.5751 \\
%     w/o Logic Regularization & 0.5748  & 0.6918  &   0.3946  &  0.5764 \\
%   \bottomrule
% \end{tabular}
% \vspace{-3mm}
% \end{table}
% \begin{table}[]
%   \caption{Variants of \shortname, where ``Feat''. short for Feature and ``Embed.'' short for Embedding. The bold font(\textbf{N}) marks the best result within a column.}
%   \label{tab:variant}
%   \centering
%   \small
%   \begin{tabular}{ll|ll|ll}
%     \toprule
%     \multicolumn{2}{c}{}&
%     \multicolumn{2}{c}{\textbf{RSC2017}}&
%     \multicolumn{2}{c}{\textbf{Taobao}} \\
%     \cmidrule(lr){3-6} 
%     & & NDCG@10 & HR@10 & NDCG@10 & HR@10 \\
%     \midrule
%     \multicolumn{2}{c|}{FENCR}& \textbf{0.5797} &  \textbf{ 0.6941}  &  \textbf{0.3996} &  \textbf{0.5837} \\
%     \midrule
%     \multirow{2}{*}{Input} & User Feat. & 0.5478 & 0.6474 & 0.3363 & 0.4991 \\
%      & Item Feat.   & 0.5389 & 0.6549  & 0.3938  & 0.5679\\ 
%     \midrule
%     \multirow{3}{*}{Weight}
%     & User Embed. & 0.5669 & 0.6862 & 0.3861 &   0.5720 \\
%     & Item Embed. & 0.5748 & 0.6899 & 0.3908 &   0.5743\\
%     &  Constant & 0.5545 & 0.6772 & 0.3773   &   0.5684 \\
%   \bottomrule
%   \vspace{-5mm}
% \end{tabular}
% \end{table}

% \subsection{Overall Performace}
% \label{sec:overall_performance}

% To answer $\boldsymbol{RQ1}$ and investigate the performances of our proposed model, we report the performance of \shortname~ and all baselines on RSC2017 and Taobao datasets in Table \ref{tab:performance_rec} on the HR@K and NDCG@K metrics. We record the mean and standard deviation values of five trials for each experiment.

% First, all methods incorporating features perform better than none-feature models, except for XGBoost on RSC2017 and FM on the Taobao dataset. The observation demonstrates the importance of incorporating content information in recommender systems.

% Second, we can see that incorporating logic properties into traditional neural recommendations benefits model performance.
% LTNRec outperforms BiasedMF+MSE. We make this comparison because since the logic loss in LTNRec is based on the MSE loss, it is unfair to compare with models using BPR loss. NCR outperforms BasiedMF and NLR. NLR is worse than BaisedMF in RSC2017, probably because NLR fails to utilize collaborative filtering signals, and mainly relies on users' interaction histories. 
% %In general, we can see a positive effect of the incorporation of logic over existing model architectures, which is consistent with the results of previous work.

% Third, for models that learn explicit logic rules in content-aware recommendation, \shortname~ with vector encoding of features outperforms NS-ICF, suggesting an essential role of probabilistic embedding as representation.
% %which is probably because that embedding vectors can learn implicit relationships between feature values compared to one-hot encoding. 
% It should be noted that although we use the same Taobao dataset as NS-ICF, the reported performance of NS-ICF differs from the original manuscript~\cite{ZhangNSICF2022}. It may be due to different data pre-processing and evaluation settings. We sample 1000 negative items in calculating metrics, while 20 negative items are sampled in the original work. The impact of sample size on model performance is also pointed out in previous work~\cite{DBLP:KDDsampleN}.

% % 我们的模型outperform了
% Last, our proposed model \shortname~ performs best among all compared models. 
% % In particular, \shortname~ significantly outperforms state-of-the-art neural logical recoomendation models and traditional feature-enhanced models. 
% In addition, \shortname~ provides additional explainability by learning logic rules, which will be demonstrated in Section \ref{sec:casestudy}.
% %The improvement implies the continuous neural reasoning methods are potential in both utilities and explainability. 
% % \begin{table}[]
% %  \vspace{-1mm}
% %   \caption{Variants of \shortname. The bold font(\textbf{N}) marks the best result within a column.}
% %   \label{tab:variant}
% %   \centering
% %   \small
% %   \begin{tabular}{l|lll}
% %     \toprule
% %     \multicolumn{1}{c}{}&
% %     \multicolumn{3}{c}{\textbf{RSC2017}}\\
% %     \cmidrule(lr){2-4} 
% %      & NDCG@5 & NDCG@10 & HR@10 \\
% %     \midrule
% %     FENCR& \textbf{0.5579}  &   \textbf{0.5797}   &  \textbf{ 0.6941}   \\
% %     \midrule
% %     U-F Only & 0.5296 & 0.5478 & 0.6474  \\
% %     I-F Only & 0.5169 & 0.5389 & 0.6549  \\ 
% %     \midrule
% %     U-S Voting & 0.5445 &  0.5669 & 0.6862 \\
% %     I-S Voting & 0.5533 &  0.5748  & 0.6899 \\
% %     C-W Voting & 0.5322 &  0.5545  & 0.6772  \\
% %     \midrule
% %     \midrule
% %     \multicolumn{1}{c}{}&
% %     \multicolumn{3}{c}{\textbf{Taobao}}\\
% %     \cmidrule(lr){2-4} 
% %      & NDCG@5 & NDCG@10 & HR@10 \\
% %     \midrule
% %     FENCR &  \textbf{0.3653} &   \textbf{0.3996}   &  \textbf{0.5837}\\
% %     \midrule
% %     U-F Only & 0.3071 & 0.3363 & 0.4991 \\
% %     I-F Only & 0.3609 & 0.3938 & 0.5679 \\
% %     \midrule    
% %     U-S Voting  & 0.3508 &   0.3861   &   0.5720\\
% %     I-S Voting & 0.3567  &   0.3908   &   0.5743\\
% %     C-W Voting & 0.3412 &   0.3773   &   0.5684\\

% %   \bottomrule
% % \end{tabular}
% % \end{table}
% \begin{table*}[]
% \centering
% \caption{Generated Decision Reasons for Four Random Selected Cases (Best Viewed in Color).}
% \vspace{-2mm}
% \label{tab:case_study}
% \begin{tabular}{cc|p{12cm}}
% \toprule
% \multicolumn{2}{c|}{\textbf{Dataset}}   & \textbf{Generated Decision Reasons with Highest Score $\mathbf{w}_i$ in Equation~\eqref{eq:aggregation_rules}} \\
% \midrule
% \multirow{4}{*}{\textbf{RSC2017}} & \multirow{2}{*}{Case \#1}  &
% \textcolor{orange}{U.CareerLevel}=Manager $\lor$
% \textcolor{blue}{U.ExperienceYears}=MoreThan20Years \\
% & &  $\lor$ \textcolor{orange}{I.CareerLevel}=Professional/Experienced $\lor$ \textcolor{red}{I.Latitude}=40 $\lor$ \textcolor{LightSkyBlue}{I.Employment}=Full-Time \\ 
% \cmidrule{2-3}
%  & \multirow{2}{*}{Case \#2} &
% \textcolor{Green}{U.ID}=259584 $\land$
% \textcolor{Violet}{U.WillingToChangeJob}=HighInterest $\land$ \textcolor{SpringGreen}{U.Premium}=Active $\land$ \textcolor{purple}{I.Country}=Germany $\land$ \textcolor{SeaGreen}{I.IsPaid}=Yes $\land$ \textcolor{Indigo}{I.Longtitude}=Null $\land$ 
% \textcolor{ProcessBlue}{I.CreateTime}=25 (Month) \\
% \midrule

% \multirow{4}{*}{\textbf{Taobao}}
%  & \multirow{2}{*}{Case \#3}  &
% \textcolor{Green}{I.ID} = 670415 $\lor$
% \textcolor{purple}{U.PriceLevel}=Medium $\lor$
% \textcolor{orange}{U.ShopLevel}=High  $\lor$ \textcolor{red}{U.UniversityStudent}=Yes  $\lor$ \\
% & &  \textcolor{ProcessBlue}{I.CategoryID}=6261 $\lor$ \textcolor{Indigo}{I.Price}=0-1000 \\ 

% \cmidrule{2-3}
%  & \multirow{2}{*}{Case \#4}  &
% \textcolor{Green}{U.ID}=36009 $\land$
% \textcolor{blue}{U.AgeLevel}=4  $\land$ \textcolor{orange}{U.ShopLevel}=High $\land$ \textcolor{red}{U.UniversityStudent}=Yes $\land$ \\
% & &   \textcolor{LightSkyBlue}{U.CityLevel}=3 $\land$ \textcolor{ProcessBlue}{I.CategoryID}=7548 \\ 

% % \multirow{3}{*}{199439} & \multirow{3}{*}{16317} &
% % \textcolor{Green}{U.ID}=199439 $\land$
% % \textcolor{Violet}{U.WillingToChangeJob}=HighInterest $\land$ \textcolor{SpringGreen}{U.Premium}=Active $\land$ \textcolor{purple}{I.Country}=Germany $\land$ \textcolor{SeaGreen}{I.IsPaid}=Yes $\land$ \textcolor{Indigo}{I.Longtitude}=Full-Time $\land$ 
% % \textcolor{ProcessBlue}{I.CreateTime}=25 (Month) & \multirow{3}{*}{0.951}\\
% \bottomrule
% \end{tabular}
% \end{table*}

% \subsection{Ablation Study and Model Variants} 
% \label{sec:ablation}

% We conduct ablation studies and explore various model variants to gain insights into the designation of our proposed approach \shortname~(\textbf{RQ2}). 
% % To answer \textbf{RQ2}, this section tests the influence of our proposed modules and the hyper-parameters. 
% First, we conduct ablation on the feature selector (w/o Feature Selector) and logic regularization term (w/o Logic Regularization). Removing the selector module results in using an all-1 $\boldsymbol{M}$ matrix without selecting various feature groups. Removing the logic regularization term suggests $\lambda_r$ in Section \ref{sec:Loss} is 0. As shown in Table \ref{tab:ablation}, the performance degradation shows the modules' effectiveness.
% Second, as shown in Table~\ref{tab:variant} we study variants of \shortname~ in the input stage (Input) and the aggregation stage (Weight). 
% In variants for the input stage, ``User Feat.'' stands for only using features on the user side, and ``Item Feat.'' stands for only using features on the item side. In both cases, user and item IDs are retained. %considering the experiment aims to explore the effect of content information in the model.
% \shortname~ outperforms both variants of using features on the single side.
% In variants for the aggregation stage, we analyze different strategies for weighting multiple rules. Instead of using a concatenation of user and item embeddings, as introduced in Equation \ref{eq:voting_function}, ``User Embed.'' refers to using the user embedding only, and ``Item Embed.'' refers to using the item embedding only. ``Constant'' refers to training a global weight shared by all with a linear layer.
% %study the effect of the personalized voting strategy in \shortname, in which four different strategies are tested for deciding the weight of different rules. The basic strategy is learning a global weight that is shared by all data using a linear layer. On this basis, the item-specific strategy refers to introducing item embedding as input when learning weights. Similarly, the user-specific strategy uses user embeddings only as input information, while the user\&item-specific strategy 
% Experiments demonstrate the benefits of introducing user-\&item-id embeddings in aggregating multiple rules.
% %the user\&item-specific strategy achieves the best performance, followed by user-specific and item-specific strategy. 
% %The results indicate the importance of using personalized weights in summing scores based on various rules. 
% % Specifically, we find a better result in using the item-specific strategy, which may imply that the importance of different rules varies especially on different items.

% \begin{figure}[htbp]
%   \vspace{-1mm}
%     \centering
% \includegraphics[width=1\linewidth]{data/r_shape_new.pdf}
%  \vspace{-2mm}
%     \caption{Parameter analysis of \#rule($N$) in each logical module.}
%     \label{fig:r_shape}
%     \vspace{-5mm}
% \end{figure}

% \subsection{Parameter Analysis}
% \label{sec:parameter_analysis}
% To further investigate the proposed model \shortname~, we conduct parameter studies on $N$, which denotes the predefined number for each type of rule.
% %   \includegraphics[width=0.6\linewidth,trim={0 0mm 0mm 0mm},clip]{data/r_logic.pdf}
% %   \caption{Parameter analysis of $\lambda_r$ on two datasets.}
% %   \label{fig:r_logic}
% % \FloatBarrier
% % \begin{figure}[htbp]
% % \vspace{-3mm}
% %   \centering
% %   % \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
% %   \includegraphics[width=1.0\linewidth,trim={0 0mm 0mm 0mm},clip]{data/r_shape.pdf}
% %   \vspace{-8mm}
% %   \caption{Parameter analysis of \#rule in each logical module.}
% %   \vspace{-5pt}
% %   \label{fig:r_shape}
% % \end{figure}
% % \FloatBarrier
% The results are shown in Figure \ref{fig:r_shape}. 
% In our model, the computational complexity is directly proportional to $N$.
% Considering both model complexity and effectiveness, we choose 16 as the best parameter for experiments and analyses.
% % U.ID

% % \begin{table}[htbp]
% %   \caption{The most \textbf{frequent} features in generated rules.}
% %   \label{tab:most_features}
% %   \centering
% %   \small
% %   \begin{tabular}{l|l}
% %     \toprule
% %     \multicolumn{2}{c}{\textbf{RSC2017}} \\
% %     %\multicolumn{2}{c}{\textbf{Least Frequent}}
% %     \midrule
% %     Feature&  Count \\
% %     \midrule
% %     UserExperienceYears & 28  \\
% %     ItemCreateTime &   27  \\
% %     UserExperienceYearsInCurrent & 27  \\
% %     \midrule
% %     \midrule
% %     \multicolumn{2}{c}{\textbf{Taobao}} \\
% %     %\multicolumn{2}{c}{\textbf{Least Frequent}}
% %     \midrule
% %      Feature  & Count \\
% %     \midrule
% %      UserPriceLevel  & 28  \\
% %      UserShopLevel  & 27  \\
% %      UserOccupation & 26 \\
% %   \bottomrule
% % \end{tabular}
% % \end{table}
% \subsection{Case Study}
% \label{sec:casestudy}
% %As we have analyzed the effect of the model, we also conduct a case study of generated rules to better understand the explainability of \shortname.
% %Since we have analyzed the utilities of the model, we would like to study and demonstrate the explainability of the model to answer \textbf{RQ3}. %Specifically, we would like to first give concrete cases for logic rule-based explanations generated by ~\shortname. Then, we statistically investigate features that make up the rules.
% % \begin{figure}
% % \vspace{-2mm}
% % \centering
% % \subfigure[RSC2017(\#rules: 32)]{
% %     \begin{minipage}[b]{0.22\textwidth}
% %     \includegraphics[width=1\textwidth,trim={7mm 7mm 15mm 13mm},clip]{data/rule_feature_distribution_recsys.png}
% %     \end{minipage}
% % }
% % \subfigure[Taobao(\#rules: 32)]{
% %     \begin{minipage}[b]{0.22\textwidth}
% %     \includegraphics[width=1\textwidth,trim={7mm 7mm 15mm 13mm},clip]{data/rule_feature_distribution_Taobao.png}
% %     \end{minipage}
% % }
% % \vspace{-2mm}
% % \caption{Number of times the feature appears in the rule.} \label{fig:count}
% % \end{figure}

% \subsubsection{Explanatation Cases}

% We demonstrate generated logic rule-based reasons for recommendation in Table \ref{tab:case_study}. The presented cases are rules with the highest scores, implying the most critical reasons for the recommendation. 
% Specifically, the scores here are the personalized weights $\mathbf{w}_i$ in Equation~\eqref{eq:aggregation_rules}.
% %These cases showcase different patterns behind recommendations.

% These cases mainly show users' basis for making positive decisions. The conjunction notation $\land$ indicates the user is more inclined to make a positive decision considering all conditions. The $\lor$ indicates that some conditions are met will cause the user to make the decision. 
% For example, in case \#1, the disjunction notation $\lor$ denotes the job applicant is an experienced management professional or someone who has worked for many years. They are preferable to click the jobs that require rich working experience. 
% In case \#2, The conjunction notation $\land$ indicates that the person who is very eager to find a job would become a premium and click on the job notice paid for by a company. 
% We further speculate that it may be difficult to find a suitable candidate for this position since it is posted for 25 months and paid for by a company.
% % because a job that has been posted for 25 months and paid for is most likely fraudulent, in order to scam users out of their clicking fees. 
% % Maybe such a rule can also fit other users simultaneously, though it only fits user 259584 in this case. 
% Case \#3 is easier to understand, which denotes that users who meet several criteria may click on a specific price item or a particular category of products.
% Case \#4 shows a personalized preference for a product with category 7548 of user 36009 with other specific features, such as the age level, shop level, university student, and city level. 
% %In case \#1m  may value the expertise of the user and the position; Case \#2 matches a paid user with strong motivation in changing jobs to a paid position; recommendation in Case \#3 is relatively concerned with price and recommendation in Case \#4 concerned with age level.
% By presenting these cases, we show the ability of \shortname~ to generate logic rule-based explanations that are readable and personalized.

% % Among these four cases, both conjunction and disjunction rules are involved and distinct feature domains are included. 

% \begin{table}[htbp]
%   \caption{The most \textbf{frequent} top-3 features in generated rules. Freq. is the abbreviation of Frequency.}
%   \label{tab:most_features}
%   \centering
%   \small
%   \begin{tabular}{ll|ll}
%     \toprule
%     \multicolumn{2}{c|}{\textbf{RSC2017}} &
%     \multicolumn{2}{c}{\textbf{Taobao}} \\
%     \midrule
%     Feature&  Freq. & Feature & Freq.\\
%     \midrule
%     UserExperienceYears & 28 & UserPriceLevel  & 28 \\
%     ItemCreateTime &   27  &  UserShopLevel  & 27  \\
%     UserExperienceYearsInCurrent & 27  & UserOccupation & 26 \\
%   \bottomrule
%    \vspace{-5mm}
% \end{tabular}
% \end{table}

% \subsubsection{Features in generated rules}% Features statistic/importance in generate rules
% We list the most frequently appearing features in Table \ref{tab:most_features} and the number of their appearance. 
% % We can find that in RSC2017, 1) the estimated number of years of work experience that the user has (UserExperienceYears), 2) the create time of items (ItemCreateTime, processed and represented in months), 3) the estimated number of years that the user is already working in current job (UserExperienceYearsInCurrent) are the three most frequent features. In Taobao, the price level of the user consumption (UserPriceLevel), the shop level of the user (UserShopLevel), whether the user is a college student (UserOccupation) are the three most frequent features.
% %This analysis derived from \shortname~ can help people gain further insight into the data.
% It seems reasonable that for the job recommendation task, the most used features are related to the users' experience. However, it is surprising that the most appeared item-related features also include \textit{ItemCreateTime}. We suppose the possible reason is that the item with longer \textit{CreateTime} may demonstrate that the corresponding job is unstable or hard to find suitable candidates. From the Taobao dataset, it is also reasonable that the features that can reflect users' consumption levels and habits occupy several frequently occurring features. 
% This analysis derived from rules generated in \shortname~ can help people gain further insight into the data.
% %The results also show that our proposed model can identify critical features in users' reasoning processes.


% % \subsubsection{Weights distribution of rules}

% % \begin{figure*}[htbp]
% % \vspace{-3mm}
% % \centering
% % \subfigure[U.ID $\land$  U.CareerLevel $\land$ U.ExperienceYears $\land$
% %  U.ExperienceYearsInCurrent 
% %  $\land$ U.WillingToChangeJob $\land$  I.CareerLevel $\land$  I.Country $\land$ I.CreateTime]{
% %     \begin{minipage}[b]{0.3\textwidth}
% %     \includegraphics[width=1\textwidth,trim={5mm 5mm 15mm 20mm},clip]{data/colored_dis_rules/colorful_dist_0.pdf}
% %     \label{fig:rule0}
% %     \end{minipage}
% % }
% % \quad
% % \subfigure[I.ID $\land$  U.Disdiscipline 
% % $\land$  U.Country $\land$  and  U.ExperienceYears $\land$  U.EducationDegree $\land$  U.WillingToChangeJob $\land$  U.Premium $\land$ I.Country and  I.Longitude $\land$  I.CreateTime]{
% %     \begin{minipage}[b]{0.3\textwidth}
% %     \includegraphics[width=1\textwidth,trim={5mm 5mm 15mm 20mm},clip]{data/colored_dis_rules/colorful_dist_1.pdf}
% %     \label{fig:rule1}
% %     \end{minipage}
% % }
% % \quad
% % \subfigure[U.ID $\land$  I.ID $\land$ U.Country $\land$  U.Region $\land$  UserExperienceEntries $\land$ U.ExperienceYears $\land$   U.ExperienceYearsInCurrent $\land$  U.WillingToChangeJob $\land$  U.Premium $\land$  I.Country $\land$  I.Longitude $\land$  I.CreateTime]{
% %     \begin{minipage}[b]{0.3\textwidth}
% %     \includegraphics[width=1\textwidth,trim={5mm 5mm 15mm 20mm},clip]{data/colored_dis_rules/colorful_dist_2.pdf}
% %     \label{fig:rule2}
% %     \end{minipage}
% % }
% % \subfigure[U.ID $\lor$  I.ID 
% % $\lor$ U.CareerLevel $\lor$  U.ExperienceEntries $\lor$  U.ExperienceYears $\lor $ U.ExperienceYearsInCurrent $\lor$  U.WillingToChangeJob $\lor$  U.Premium $\lor$  I.Latitude $\lor$  I.Longitude $\lor$  I.CreatedTime]{
% %     \begin{minipage}[b]{0.3\textwidth}
% %     \includegraphics[width=1\textwidth,trim={5mm 5mm 15mm 20mm},clip]{data/colored_dis_rules/colorful_dist_3.pdf}
% %     \label{fig:rule3}
% %     \end{minipage}
% % }
% % \quad
% % \subfigure[U.Career $\lor$  U.ExperienceYears $\lor$  I.Career $\lor$  I.Latitude $\lor$  I.Employment]{
% %     \begin{minipage}[b]{0.3\textwidth}
% %     \includegraphics[width=1\textwidth,trim={5mm 5mm 15mm 20mm},clip]{data/colored_dis_rules/colorful_dist_4.pdf}
% %     \label{fig:rule4}
% %     \end{minipage}
% % }
% % \quad
% % \subfigure[U.Career $\lor$  U.ExperienceYears $\lor$  I.CareerLevel $\lor$  I.Latitude $\lor$  I.Employment]{
% %     \begin{minipage}[b]{0.3\textwidth}
% %     \includegraphics[width=1\textwidth,trim={5mm 5mm 15mm 20mm},clip]{data/colored_dis_rules/colorful_dist_5.pdf}
% %     \label{fig:rule5}
% %     \end{minipage}
% % }
% % \caption{Cases for the voting weights distribution of different rules in RSC2017, where U.x represents feature of the user, I.x represents feature of the item. The x-axis presents the voting weight and the y-axis presents the probability density over all data.} \label{fig:weight_distribution}
% % \vspace{-3mm}
% % \end{figure*}

% % \begin{figure}[htbp]
% % \vspace{-2mm}
% %   \centering
% %   % \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
% %   \includegraphics[width=1.1\linewidth,trim={50mm 0mm 20mm 0mm},clip]{data/distribution_all_rules.pdf}
% %   \caption{The effect of three different rules on 500 sampled data points.}
% %   \label{fig:all_dist}
% % \end{figure}

% % As we have introduced, the weights of generated rules in prediction are customized according to the user and item embedding, so we are interested in looking further at the weight distribution of the rules over all data to investigate the effect of the rules in the inference process. 

% % In Figure \ref{fig:weight_distribution}, we illustrate six rules with their weight distribution on RSC2017 as an example. Among these rules, there are cases with user id, cases with item id, cases that contain both and include neither. The figure indicates that distinct rules exhibit disparate weight distributions. The rule in Figure \ref{fig:rule0} (referred to as rule\#a) constantly maintains a high weight across all instances. The rule in Figure \ref{fig:rule1} (referred to as rule\#b) bears substantial weight in a large portion of data, and is also important in another part, but may not be critical. For rules in Figure \ref{fig:rule2} (referred to as rule\#c) and Figure \ref{fig:rule3} (referred to as rule\#d), they are effective on parts of the data, while carrying relatively less weight on another segment. The rule in Figure \ref{fig:rule4} (referred to as a rule \#e) is limited to certain data, while it may not be effective on others. The rule in Figure \ref{fig:rule5} (referred to as rule\#f) appears to have minimal impact on the inference process. 
% % %This finding shows the variation in the role that our learned rules play in the inference process.
% % These observations demonstrate the diversity in the functions that our acquired rules perform.

% % \begin{figure}[htbp]
% % \vspace{-2mm}
% %   \centering
% %   % \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
% %   \includegraphics[width=0.6\linewidth,trim={0mm 0mm 0mm 0mm},clip]{data/3d.pdf}
% %   \vspace{-9mm}
% %   \caption{The effect of three different rules on 500 sampled data points.}
% %   \vspace{-5pt}
% %   \label{fig:coverage_3d}
% % \end{figure}


% % \begin{figure*}[htb]
% % \centering
% % \vspace{-3mm}
% % \subfigure[Collaboration of Rule$\#$b $\&$ Rule$\#$c]{
% %     \begin{minipage}[b]{0.31\textwidth}
% %     \includegraphics[width=1\textwidth]{data/case2d_bc.pdf}
% %     \label{fig:rulebc}
% %     \end{minipage}
% % }
% % \subfigure[Collaboration of Rule$\#$b $\&$ Rule$\#$e]{
% %     \begin{minipage}[b]{0.31\textwidth}
% %     \includegraphics[width=1\textwidth]{data/case2d_be.pdf}
% %     \label{fig:rulebe}
% %     \end{minipage}
% % }
% % \subfigure[Collaboration of Rule$\#$c $\&$ Rule$\#$e]{
% %     \begin{minipage}[b]{0.31\textwidth}
% %     \includegraphics[width=1\textwidth]{data/case2d_ce.pdf}
% %     \label{fig:rulece}
% %     \end{minipage}
% % }
% % \caption{Collaboration of three rules on 500 samples.} \label{fig:coverage}
% % \vspace{-8mm}
% % \end{figure*}

% % \subsubsection{Collaboration of rules}
% % While we have explored the weight distribution of several rules separately, we aim to further investigate the collaborations between rules. For example, are several rules in effect simultaneously, or do different rules dominate different data? To answer these questions, for Rule\#b, Rule\#c and Rule\#e in Figure \ref{fig:weight_distribution},
% % we plot the weight of each pair of rules on 500 samples in Figure \ref{fig:coverage}. Specifically, each scatter plot displays the joint distribution of weights on two rules. 
% % %The scatter plot is shown in Figure \ref{fig:coverage_3d}, 
% % In Figure \ref{fig:rulebc}, we can obsearve a proportional trend in weights of the two rules, while Figure \ref{fig:rulebe} and \ref{fig:rulece} indicate an inverse correlation relationship between the two variables.
% % This demonstrates the diversity in collaboration of different rules. Some rules tend to operate in concert, and in other cases, some rules can cover situations that are not covered by the remaining ones.

% %in which we can observe a tendency for the weights of rules \#b and \#c to increase at points where the weight of rule \#d is low. This shows that while the effect of all three rules is evident on a small amount of data, in more cases, different data points are dominated by different rule sets.

% % \subsection{手动指定规则实验}

==> 5-conclusion.tex <==
\section{Conclusion}
% 我们的工作不是一个关于方法设计，只是一个可行性的证明
% 要呼应一下意义，呼应contribution，不能只说做了什么，解决了什么挑战
\label{sec:conclusion}
In this paper, we propose \shortname, which learns logical rules as explanations and feature embedding for representation.
% The model is trained in an end-to-end manner.
% To the best of our knowledge, we are the first to incorporate dense feature embeddings in neural logical recommendations methods.
We design novel neural logical modules that represent conjunction and disjunction to better learn feature interactions in logic operations on vectors.
The inference procedure of \shortname~ can be interpreted into logical rules.
Experiments show \shortname~ outperforms previous logic-enhanced recommendation models while being able to provide rule-based reasons for the results.
We believe that using logic rules as explanations is a topic worth exploring. As explanations in the form of logic rules are easy to understand and modify, they are more stable and controllable when supporting downstream applications.
In the future, we will further study the potential downstream tasks of generated rules, including providing guidance to feature engineering and collaborating with language models for generating more persuasive texts.

% Our work is still limited. A question worth considering is whether the learned rules conform to human cognitive processes.
% To address this issue, additional supervision could be added to align the learning of logic rules towards human decision process.

% 容易引入其他信息；拓展到非recommendation的工作上；
